ROS2-Based Simulation Framework for Cyberphysical Security Analysis of UAVs

We present a new simulator of Uncrewed Aerial Vehicles (UAVs) that is tailored to the needs of testing cyber-physical security attacks and defenses. Recent investigations into UAV safety have unveiled various attack surfaces and some defense mechanisms. However, due to escalating regulations imposed by aviation authorities on security research on real UAVs, and the substantial costs associated with hardware test-bed configurations, there arises a necessity for a simulator capable of substituting for hardware experiments, and/or narrowing down their scope to the strictly necessary. The study of different attack mechanisms requires specific features in a simulator. We propose a simulation framework based on ROS2, leveraging some of its key advantages, including modularity, replicability, customization, and the utilization of open-source tools such as Gazebo. Our framework has a built-in motion planner, controller, communication models and attack models. We share examples of research use cases that our framework can enable, demonstrating its utility.

==> tables/drone-simulators.tex <==
\begin{table*}[!t]
    \caption{Comparison of Drone Simulators}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \textbf{Simulator} & \textbf{ROS Support} & \textbf{Language Support}
                           & \textbf{Sensors}     & \textbf{Physics engine}   & \textbf{License}
        \\
        \hline
        Gazebo             & \checkmark           & C++, Python
                           & GPS, IMU, Camera     & Multiple                  & Open Source
        \\
        \hline
        MORSE              & \checkmark           & Python
                           & Full                 & Bullet                    & Open Source
        \\
        \hline
        CoppeliaSim        & \checkmark           & C++, Python, Lua
                           & Various sensors      & Multiple                  & Proprietary
        \\
        \hline
        Webots             & \checkmark           & C, C++, Python
                           & Lidar, Camera, IMU   & ODE                       & Proprietary
        \\
        \hline
    \end{tabular}
\end{table*}

